Selective Annotation Makes Language Models Better Few-Shot Learners

Many recent approaches to natural language tasks are built on the remarkable abilities of large language models. Large language models can perform in-context learning, where they learn a new task from a few task demonstrations, without any parameter updates. This work examines the implications of in-context learning for the creation of datasets for new natural language tasks. Departing from recent in-context learning methods, we formulate an annotation-efficient, two-step framework: selective annotation that chooses a pool of examples to annotate from unlabeled data in advance, followed by prompt retrieval that retrieves task examples from the annotated pool at test time. Based on this framework, we propose an unsupervised, graph-based selective annotation method, voke-k, to select diverse, representative examples to annotate. Extensive experiments on 10 datasets (covering classification, commonsense reasoning, dialogue, and text/code generation) demonstrate that our selective annotation method improves the task performance by a large margin. On average, vote-k achieves a 12.9%/11.4% relative gain under an annotation budget of 18/100, as compared to randomly selecting examples to annotate. Compared to state-of-the-art supervised finetuning approaches, it yields similar performance with 10-100x less annotation cost across 10 tasks. We further analyze the effectiveness of our framework in various scenarios: language models with varying sizes, alternative selective annotation methods, and cases where there is a test data domain shift. We hope that our studies will serve as a basis for data annotations as large language models are increasingly applied to new tasks. Our code is available at https://github.com/HKUNLP/icl-selective-annotation.

==> text/abstract-old.tex <==
\begin{abstract}
%\tao{
%maybe highlighting the following points in abstract and introduction? 
%1) Unlike LM fine-tuning paradigm~\citep{darcy2022limitations}, selecting data to annotate is very important for few-shot in-context learning, which has been overlooked in recent studies. 
%2) Better few-shot in-context learning prompting via selecting diverse and representative examples to annotate?
%3) In-context learning with wisely-selected examples is a much better few-shot practice than other methods including fine-tuning?
%}
%\jungo{we haven't decided what name we use for the first step. Use the command, \\firststep so we can change later.}

\textit{In-context learning} is a new, promising paradigm in natural language processing that allows a language model to learn a new task from a few task demonstrations \emph{without} any parameter updates.
%to generate an answer for unseen test input.
%At the core of in-context learning is selection of in-context, demonstration examples that provide a few input-output pairs upon which the language model condition its generation.
Recent work proposed effective methods to retrieve these demonstrations from the training data to create a prompt for each individual test input.
%\tao{is it better to combine the previous two sentences? emphesis on prompt retrieval too much?}
These methods, however, implicitly assume access to the \emph{full, large}, \emph{labeled} training data, which is expensive to obtain.
%diverging from the original few-shot learning scheme.
%; while each test instance only requires a few labeled examples for prompting, different test instances inrequire labeled examples to be retrieved.
%To achieve realistic few-shot in-context learning,
%\tao{this motivation looks a bit weak. how about: to study the best "real" few-shot practice: including ICL and FT...}, 
%we formulate a two-step framework: some examples are chosen to be labeled (sample selection), and a subset of them is retrieved for every test instance (prompt retrieval) \tao{deemphasize on two-step framework? looks more like sample selection . re-framing it?}.
%\rui{We should be very direct about our two-step framework and its implications on "annotation cost". Otherwise, readers can easily get lost. So I add:}
% To carefully study the annotation cost required by in-context learning, we formulate a general two-step framework that decouples \firststep and prompt retrieval.
In this paper, we show the importance of \emph{\firststep} for in-context learning, which has been overlooked in recent work. 
\luke{Need to define what \firststep actually is a bit more directly? Assume access to possible inputs and decide which to annotate without knowing their outputs? }
To quantify the annotation cost for in-context learning, we formulate a two-step framework: \firststep that chooses a pool of examples to annotate and prompt retrieval that retrieves demonstration examples from the pool.
% In this paper, we formulate a two-step in-context learning framework that decouples \firststep and prompt retrieval.
% We show the importance of \firststep for in-context learning, which has been overlooked in recent work.
% Under this framework, the total annotation cost is the number of labeled retrieval targets.
Our extensive experiments on 10 diverse datasets on 9 distinct tasks demonstrate that selecting diverse, representative examples improves in-context learning by a large margin, under the same small annotation budgets. 
% (5.8\% and 5.2\% absolute gains \tao{Hongjin TODO: report relative
% improvement} on average for 18 and 100 annotation sizes respectively).
On average, it achieves a 13.0\% relative gain for a budget of 18 annotated examples and a 10.4\% relative gain for 100 annotated examples.
% (13.0\% and 10.4\% relative gains on average for 18 and 100 annotation sizes respectively).
It also yields similar performance with 10-100x less annotation cost, compared to state-of-the-art finetuning methods.
% \tao{too much about the two-step method. no need that many annotated data, ICL with 100 performs similar to 10k...? if use fixed 18 examples, select vs random > 10\%. Unlike LM fine-tuning paradigm, sample selection is very important for few-shot in-context learning, which has been overlooked in recent studies. the best few-shot performance, no need to annotate that many for ICL}
%Our extensive experiments on diverse 10 datasets demonstrate that in-context learning outperforms state-of-the-art finetuning methods by \jungo{Hongjin's TODO} on average, under the same annotation budget.
%Further, in-context learning achieve similar performance to the finetuning models with 5-8x less annotation cost. 
%\rui{These two sentences are not very clear: 1st: "ICL outperforms SOTA finetuning" vs 2nd:"ICL similar to finetuning with less annotation cost". We can merge them to deliver a clear and strong message. It is also good to have concrete numbers, e.g., resulting in up to 5-8x reduction in annotation cost without performance loss.}
%Through this analysis, we find that a small number of \emph{carefully-selected} examples suffice to perform (e.g., 100 training examples) on par with the full training data, across 10 diverse tasks in natural language processing.
Extensive analyses show that our method improves in-context learning across language models with varying sizes and outperforms various \firststep methods \rui{Not very clear about "various selective annotation methods" as we didn't mention vote-k and other baselines in abstract.}.
Furthermore, the improvement is even more pronounced when there is a domain shift in the evaluation data.
%\tao{a better phrase for \firststep? \rui{Is "coreset selection" better?}}
%\weijia{People mainly use ICL for few-shot learning and may care more about few-shot setting. Maybe we could emphasize that even in true few-shot setting without prompt retrieval (training data pool size = number of ICL examples), our method is also very effective. }
% \footnote{Our code is available at \url{}.}

\begin{figure}[t!]
\centering
    \includegraphics[width=0.98\textwidth]{images/main_plot.pdf}
\caption{Comparisons between the in-context learning and finetuning paradigms over varying annotation budgets on three various tasks (more experiments over 10 datasets in Tab.~\ref{tab:main_results}). %(i.e., the size of the labeled samples, $|\mathcal{L}|$)
Four configurations are presented: finetuning with examples that are randomly selected (FT-random) or selected by our \firststep vote-k method (\S\ref{sec:sample_selection_method}; FT-select) and in-context learning with random selection (ICL-random) and vote-k selection (ICL-select).
Detailed experimental details will be discussed in \S\ref{sec:in-context_finetuning}.
Unlike finetuning paradigm, \firststep largely improves the in-context learning performance compared to random selection even when the annotation budget is 18.
In-context learning with wisely-selected labeled samples is a much better few-shot practice than other methods.
\tao{to add: 0. more general overall caption 0.5 hellawag/mrpc gpt3; gpt3 1. fully ft performance; 2. icl retrieving from full training; 3. adding a conclusion in the caption. 4. mentioning which model is used for ICL and fine-tuning. 5. updating the plot for final ICL models. 6. one single horizontal legend; axis labels. 7. mention we did 10 datasets. 8. task -> category}
\tao{it would be nice to show GPT-J/XNeo (5x smaller model size) with wisely selected examples outperforms GPT-3 with random annotated examples!}
\rui{0. I still believe it is very important to show figure 1 right here, but let's provide enough context for readers to understand it. 1. Let's flip the order of methods in legend to align with the curves. 2. One copy of legend is fine outside of the three plots. 3. Let's stretch the horizontal axis to fit textwidth? 4. Is it better to use the same vertical axis range? 5. Is it possible to use orange color for our methods as orange is more noticeable? 6. The current figure/caption doesn't show which language models we use. Is it GPT-3 or something else?}
}
\label{fig:main_results}
\end{figure}

\end{abstract}


==> text/intro-old.tex <==
\section{Introduction}
% \begin{figure}[t!]
% \centering
%     \includegraphics[width=0.98\textwidth]{images/main_plot.pdf}
% \caption{Comparisons between the finetuning and in-context learning paradigms over varying annotation budgets (i.e., the size of the labeled samples, $|\mathcal{L}|$). Four configurations are presented: finetuning with examples that are randomly selected (FT-random) or selected by vote-k (\S\ref{sec:sample_selection_method}; FT-vote-k) and in-context learning with random selection (ICL-random) and vote-k selection (ICL-vote-k).
% The two in-context learning settings both use similarity-based prompt retrieval (\S\ref{sec:prompt_retrieval_method}).
% When $|\mathcal{L}|=18$, in-context learning does \emph{not} require any prompt retrieval because all 18 examples can be fit as input to the language model. 
% % \rui{Not sure if this sentence is important to add here.}
% The two random selection settings plot the average from three trials (the bands show the ranges).
% More details will be discussed in \S\ref{sec:in-context_finetuning}.
% % \jungo{Hongjin's TODO: clean up notations/legends. Bigger fonts. Add axis labels. (Accuracy, annotation size etc) }
% % \rui{Hongjin's TODO: Please use better color choices: e.g., from \url{https://colorbrewer2.org/\#type=diverging\&scheme=PuOr\&n=4}. Please reiterate our main message from this figure.}
% \tao{to add: 0. hellawag/mrpc gpt3; gpt3 1. fully ft performance; 2. icl retrieving from full training; 3. adding a conclusion in the caption. 4. mentioning which model is used for ICL and fine-tuning. 5. updating the plot for final ICL models. 6. one single horizontal legend; axis labels. 7. task -> category}
% % \rui{We use SST-5 and NQ results in our intro; shall we include their figures here?}
% % \tianlu{I would recommend adding a conclusion in the caption.}
% % \jungo{Yes, let's do it once we finalize the plots.}
% }
% % \hongjin{will modify this figure after deciding the model for ICL (GPT-neo-20b, Codex, OPT, etc.)}
% % \weijia{Maybe it is worth mentioning which model is used for ICL and fine-tuning}
% \label{fig:main_results}
% \end{figure}
%Large language models (e.g., GPT-3; \citealp{gpt3})  
\textit{In-context learning} is a new paradigm in natural language processing where large pretrained language models (e.g., GPT-3; \citealp{gpt3}) learn a new task by conditioning text generation upon a \emph{prompt} with a few in-context examples (i.e., task input-output demonstrations).
It thus requires no updates to the model parameters.
% In-context learning is an attractive alternative to supervised finetuning, as it allows the large language model to avoid expensive finetuning and to adapt to new scenarios with a few in-context examples for prompting \citep{prompt_survey}. 
A flurry of recent work \interalia{gpt3,liu-etal-2022-makes,hu_dialogue} proposed methods for in-context learning that can achieve competitive performance to finetuning in many tasks, including question answering \citep{berant-etal-2013-semantic,joshi-etal-2017-triviaqa,kwiatkowski2019natural}, sentiment analysis \citep{socher-etal-2013-recursive}, and semantic parsing~\citep{Rajkumar2022EvaluatingTT}.
%, and dialogue state tracking \citep{budzianowski-etal-2018-multiwoz}.
%

One crucial limitation of these in-context learning methods is that their performance heavily depends on the choice (and even the order) of in-context examples in the prompt \citep{liu-etal-2022-makes,hu_dialogue,lu-etal-2022-fantastically,rubin2022}.
In particular, recent work has shown that the performance substantially improves when similar (under some embedding function) examples are retrieved as in-context examples for each test input \citep{liu-etal-2022-makes}.
However, most recent work assumes that a large set of annotated training examples is available to be used as possible in-context examples.
%diverging from the original few-shot scheme in terms of the required annotation cost \citep{gpt3}.
% It is not clear which examples should be selected to annotate to make in-context learning work for new tasks that a large annotated dataset is not available.
% Even for tasks with a large labeled training data, how many labeled examples are really needed to achieve decent in-context learning performance has been also understudied. 
Each test sample only requires a few in-context examples in its prompt, but they need to be retrieved individually with their associated annotations.

In this work, we present in-depth studies on the effect of \emph{\firststep} for in-context learning.
We investigate how to select examples to annotate to make in-context learning work better on new tasks for which a large annotated dataset is not available.
Even for tasks with large labeled training sets, we study how many labeled examples are really needed to achieve strong in-context learning performance. 
We establish a two-step framework that quantifies the annotation cost for in-context learning as shown in Fig.\ \ref{fig:framework}: the first step is \textit{\firststep} that picks instances to get annotated, and the second step is \textit{prompt retrieval} that retrieves in-context examples for each test instance from the candidate pool obtained by the first step. 
The total annotation budget is the number of candidates selected in the first step, and the second step is bounded by the number of examples that can fit as input to a language model.
% the number of retrieval targets corresponds to the annotation budget.
% Under this framework, prior methods that select in-context examples from all training data (e.g., \citealp{liu-etal-2022-makes,hu_dialogue}) can be viewed as a special case where the annotation budget is the same as the size of the original training data, which is generally very large (e.g., 10K). 
% \tao{more our findings and result analysis instead of the framework}

% Our framework \tao{check} enables us to systematically compare the annotation cost for in-context learning methods.
We find that, as shown in Fig.\ \ref{fig:main_results}, \firststep largely improves in-context learning over random selection.
This is in contrast with finetuning, where we cannot see its effectiveness over random selection. %\citep{darcy2022limitations}. 
% To reduce the annotation cost, we propose an \firststep method, vote-k, that selects a diverse and representative candidate set to annotate, based on the graph structure of unlabeled samples (\S\ref{sec:sample_selection_method}).
Our extensive experiments over 10 datasets across diverse tasks (Tab.~\ref{tab:main_results}) demonstrate that our proposed \firststep method, vote-k (\S\ref{sec:sample_selection_method}), substantially improves the in-context learning performance through balancing the diversity and representativeness of selected samples. % (\S\ref{sec:div_rep_analysis}).
For instance, voke-k, combined with a similarity-based prompt retrieval method \citep{liu-etal-2022-makes,rubin2022}, improves in-context learning by 5.2\% on average when the annotation size is 100.
Surprisingly, with an annotation budget of 18 examples where fixed in-context examples are used for all testing instances (no prompt retrieval is performed), in-context learning with vote-k still outperforms the random selection baseline by 5.8\% on average.
% 7.8 accuracy points on the SST-5 sentiment analysis task \citep{socher-etal-2013-recursive} and 9.9 points on the GeoQuery semantic parsing task \citep{geoquery96}.

%Furthermore, we show that wisely-selected annotated examples make in-context learning better and robust.
Our framework provides a better few-shot practice with 5-100x less annotation cost for new natural language tasks.
As shown in Tab.~\ref{tab:main_results}, in-context learning with 18 examples selected by vote-k achieves higher performance than with 100 randomly selected examples on 7 out of 10 tasks, with 5-10x less annotation cost.
It also outperforms the state-of-the-art few-shot finetuning methods by a large margin (Fig.\ \ref{fig:main_results}) \chen{check: are we using sota few-shot finetuning methods or just plain finetuning?} and requires an order of magnitude (usually 10-100x) less annotations for similar performance (\S\ref{sec:in-context_finetuning}).
By labeling diverse and representative data as the fixed in-context examples or the prompt retrieval pool, in-context learning prompting becomes much more stable and robust. 
%Moreover, Fig.\ \ref{fig:main_results} indicates that
Moreover, in-context learning quickly (100 or 300 samples are annotated) converges to decent performance when vote-k \firststep is applied, indicating that large training data (e.g., 10K) is not necessary for in-context learning.


Not only can our framework achieve consistent improvement over language models with varying sizes (2-175B parameters), we can see larger improvements when there is a domain shift between training and test data (e.g., text from different Amazon users; \citealp{wilds}).
Our analysis illustrates that vote-k selection is able to find a balanced middle ground between diversity and representativeness, which outperforms all other annotation or active learning methods in the in-context learning paradigm.
As in-context learning has been applied to a wide range of natural language processing applications, we hope that our annotation-efficient framework will provide useful guidance for both researchers and practitioners of in-context learning.

\rui{The last three paragraphs in intro contains a lot of messages which is a bit unorganized, e.g., we jump back and forth from Fig 1 and Tab 1, making it hard for readers parse. How about we first list several key findings in plain English, and then present evidence for each?}
